Capital growth since the 19th century

We argued in an earlier paper (Getty and Tkachenko 2025b), from data reported for net saving and market-value capital by 94 nations over the period 1980-2021, that net saving has had little or no effect on capital growth at the global scale. Here we extend the study backward to the earliest year, in each country, for which those data have been reported or reconstructed. We find a still smaller margin of possibility (1.6% versus 6.4%) of contribution of net saving to capital growth at the collective scale. We also propose and defend an alternative explanation of capital growth, and suggest a larger role for the cash flow concept in economic analysis.

==> tables/tbl-4.tex <==
\centering
\begin{tabularx}{\columnwidth}{lcc}
   Regression of $s^*$ on \(g(K)\)   & 0.1047$^{***}$\\   
                                     & (0.0106)\\   
   Observations                      & 2,744\\  
   R$^2$                             & 0.68143\\  
   Within R$^2$                      & 0.14490\\  
    \\
   Year fixed effects                & $\checkmark$\\   
   Country fixed effects             & $\checkmark$\\   
\end{tabularx}
   \label{tbl-4}


==> tables/tbl-5.tex <==
\begin{table}[pos=h]
\caption{Country-level summary of $\frac{s^*}{g(K)}$ in the current draft sample. Screen = 0.01. Period reports unscreened country coverage in the analysis file; number of years clearing screen shown in ()}\label{tbl-5}%
\hrule
\makebox[\textwidth][c]{%
{\centering

\begin{tabular}{llrr} Armenia & 1991 - 2022 (29) & -0.04\\
Aruba & 1996 - 2022 (25) & 0.19\\
Australia & 1960 - 2022 (54) & 0.42\\
Austria & 1996 - 2022 (23) & 0.75\\
Azerbaijan & 1991 - 2022 (30) & 0.40\\
\addlinespace
Bahrain & 2009 - 2022 (12) & 0.19\\
Belarus & 1991 - 2022 (30) & 0.19\\
Belgium & 1986 - 2022 (29) & 0.78\\
Bolivia & 1998 - 2022 (23) & 0.29\\
Botswana & 1990 - 2022 (31) & 0.67\\
\addlinespace
Brazil & 1996 - 2022 (20) & 0.28\\
British Virgin Islands & 1996 - 2022 (25) & 0.43\\
Bulgaria & 1996 - 2022 (23) & 0.40\\
Burkina Faso & 2000 - 2022 (21) & 0.32\\
Cameroon & 1994 - 2022 (24) & 0.51\\
\addlinespace
Canada & 1962 - 2022 (53) & 0.60\\
Cape Verde & 2008 - 2022 (13) & 0.22\\
Chile & 1997 - 2022 (23) & 0.47\\
China & 1993 - 2022 (30) & 0.68\\
Colombia & 1995 - 2022 (27) & 0.28\\
\addlinespace
Costa Rica & 2013 - 2022 (8) & 0.56\\
Croatia & 1996 - 2022 (23) & 0.04\\
Curaçao & 2001 - 2022 (20) & 0.54\\
Cyprus & 1996 - 2022 (22) & 0.14\\
Czechia & 1991 - 2022 (26) & 0.17\\
\addlinespace
Côte d’Ivoire & 1990 - 2022 (32) & 0.44\\
Denmark & 1982 - 2022 (40) & 0.33\\
Dominican Republic & 1992 - 2022 (28) & 0.31\\
Ecuador & 2008 - 2022 (15) & 0.24\\
Egypt & 1997 - 2022 (22) & 0.41\\
\addlinespace
El Salvador & 2015 - 2022 (7) & -0.33\\
Estonia & 1995 - 2022 (27) & 0.47\\
Finland & 1981 - 2022 (36) & 0.43\\
France & 1871 - 2022 (124) & 0.57\\
Germany & 1871 - 2022 (119) & 0.62\\
\addlinespace
Greece & 1996 - 2022 (24) & 0.13\\
Guatemala & 2002 - 2022 (19) & -0.57\\
Guinea & 2004 - 2022 (19) & 0.67\\
Honduras & 2001 - 2022 (16) & -0.09\\
Hong Kong & 1981 - 2022 (41) & 0.44\\
\addlinespace
Hungary & 1996 - 2022 (23) & 0.27\\
Iceland & 2001 - 2022 (19) & 0.21\\
India & 2000 - 2022 (23) & 0.52\\
Indonesia & 2017 - 2022 (5) & 0.06\\
Iran & 1997 - 2022 (20) & 0.53\\
\addlinespace
Ireland & 1996 - 2022 (25) & 0.53\\
Israel & 1996 - 2022 (25) & 0.37\\ \end{tabular}
}

{\centering
\begin{tabular}{llrr} Italy & 1981 - 2022 (35) & 0.14\\
Japan & 1981 - 2022 (28) & 0.21\\
Kazakhstan & 1991 - 2022 (29) & 0.45\\
Kuwait & 2003 - 2022 (18) & 1.34\\
Kyrgyzstan & 1991 - 2022 (31) & -0.21\\
\addlinespace
Latvia & 1995 - 2022 (26) & -0.01\\
Lithuania & 1996 - 2022 (25) & 0.22\\
Luxembourg & 1996 - 2022 (24) & 0.62\\
Malaysia & 2007 - 2022 (16) & 1.05\\
Malta & 1996 - 2022 (24) & 0.62\\
\addlinespace
Mauritius & 2014 - 2022 (8) & 0.01\\
Mexico & 1994 - 2022 (25) & 0.28\\
Moldova & 1990 - 2022 (31) & -0.28\\
Mongolia & 2006 - 2022 (15) & 0.27\\
Morocco & 1999 - 2022 (22) & 0.62\\
\addlinespace
Netherlands & 1981 - 2022 (38) & 0.52\\
New Zealand & 1987 - 2022 (32) & 0.57\\
Nicaragua & 2007 - 2022 (14) & 0.14\\
Niger & 1996 - 2022 (27) & 0.25\\
Norway & 1979 - 2022 (42) & 0.90\\
\addlinespace
Peru & 2008 - 2022 (15) & 0.46\\
Philippines & 1994 - 2022 (28) & 1.00\\
Poland & 1992 - 2022 (30) & 0.34\\
Portugal & 1996 - 2022 (22) & 0.03\\
Qatar & 2002 - 2022 (20) & -0.31\\
\addlinespace
Romania & 1990 - 2022 (30) & -0.12\\
Russia & 1996 - 2022 (22) & 0.31\\
Saudi Arabia & 2003 - 2022 (17) & 0.61\\
Senegal & 2015 - 2022 (8) & 0.12\\
Serbia & 1998 - 2022 (25) & -0.11\\
\addlinespace
Slovakia & 1993 - 2022 (24) & 0.15\\
Slovenia & 1996 - 2022 (26) & 0.44\\
South Africa & 1996 - 2022 (18) & 0.33\\
South Korea & 1971 - 2022 (51) & 0.54\\
Spain & 1996 - 2022 (22) & 0.32\\
\addlinespace
Sweden & 1951 - 2022 (64) & 0.71\\
Switzerland & 1991 - 2022 (24) & 0.42\\
Trinidad \& Tobago & 2000 - 2022 (22) & 0.01\\
Tunisia & 1993 - 2022 (27) & -0.01\\
Turkey & 2010 - 2022 (13) & 1.15\\
\addlinespace
USA & 1871 - 2022 (142) & 0.55\\
Ukraine & 1990 - 2022 (30) & 0.08\\
United Kingdom & 1856 - 2022 (142) & 0.43\\
Uruguay & 2017 - 2022 (6) & 0.63\\
Uzbekistan & 2011 - 2022 (12) & 0.12\\
\addlinespace
Vanuatu & 2002 - 2022 (19) & 0.28\\
Venezuela & 1998 - 2022 (22) & 0.20\\ \end{tabular}

}
}
\hrule
\begin{flushleft}
\footnotesize \emph{Note:} This table is based on observations with $|g(K)| > 0.01$ in the current analysis file.
\end{flushleft}
\end{table}

==> tables/tbl-country_series_coverage.tex <==
\begin{table}[H]
\caption{Coverage of the underlying series by country in the raw cleaned WID file before the analysis-sample filter. This table is not screened. Each entry reports first year, last year, and number of non-missing observations.}\label{tbl-country-series-coverage}
\hrule
\centering
\begin{tabularx}{\textwidth}{lXXXX}
\toprule
Country & Consumption & Savings & Capital & GDP\\
\midrule
Armenia & 1990 - 2025 (36) & 1990 - 2025 (36) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Aruba & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Australia & 1959 - 2025 (67) & 1959 - 2025 (67) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Austria & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Azerbaijan & 1990 - 2025 (36) & 1990 - 2025 (36) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Bahrain & 2008 - 2025 (18) & 2008 - 2025 (18) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Belarus & 1990 - 2025 (36) & 1990 - 2025 (36) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Belgium & 1985 - 2025 (41) & 1985 - 2025 (41) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Bolivia & 1997 - 2025 (29) & 1997 - 2025 (29) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Botswana & 1989 - 2025 (37) & 1989 - 2025 (37) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Brazil & 1995 - 2025 (31) & 1995 - 2025 (31) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
British Virgin Islands & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Bulgaria & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1924 - 2025 (102)\\
Burkina Faso & 1999 - 2025 (27) & 1999 - 2025 (27) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Cameroon & 1993 - 2025 (33) & 1993 - 2025 (33) & 1980 - 2025 (46) & 1945 - 2025 (81)\\
Canada & 1961 - 2025 (65) & 1960 - 2025 (66) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Cape Verde & 2007 - 2025 (19) & 2007 - 2025 (19) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Chile & 1996 - 2025 (30) & 1996 - 2025 (30) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
China & 1992 - 2025 (34) & 1978 - 2025 (48) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Colombia & 1994 - 2025 (32) & 1994 - 2025 (32) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Costa Rica & 2012 - 2025 (14) & 2012 - 2025 (14) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Croatia & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1967 - 2025 (59)\\
Curaçao & 2000 - 2025 (26) & 2000 - 2025 (26) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Cyprus & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Czechia & 1990 - 2025 (36) & 1990 - 2025 (36) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Côte d’Ivoire & 1989 - 2025 (37) & 1989 - 2025 (37) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Denmark & 1981 - 2025 (45) & 1981 - 2025 (45) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Dominican Republic & 1991 - 2025 (35) & 1991 - 2025 (35) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Ecuador & 2007 - 2025 (19) & 2007 - 2025 (19) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Egypt & 1996 - 2025 (30) & 1996 - 2025 (30) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
El Salvador & 2014 - 2025 (12) & 2014 - 2025 (12) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Estonia & 1994 - 2025 (32) & 1994 - 2025 (32) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Finland & 1975 - 2025 (51) & 1975 - 2025 (51) & 1980 - 2025 (46) & 1921 - 2025 (105)\\
France & 1950 - 2025 (76) & 1896 - 2025 (130) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Germany & 1970 - 2025 (56) & 1950 - 2025 (76) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Greece & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1948 - 2025 (78)\\
Guatemala & 2001 - 2025 (25) & 2001 - 2025 (25) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Guinea & 2003 - 2025 (23) & 2003 - 2025 (23) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Honduras & 2000 - 2025 (26) & 2000 - 2025 (26) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Hong Kong & 1961 - 2025 (65) & 1970 - 2025 (56) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Hungary & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1913 - 2025 (113)\\
Iceland & 2000 - 2025 (26) & 2000 - 2025 (26) & 1980 - 2025 (46) & 1960 - 2025 (66)\\
India & 1999 - 2025 (27) & 1951 - 2025 (75) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Indonesia & 2016 - 2025 (10) & 2016 - 2025 (10) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Iran & 1996 - 2025 (30) & 1996 - 2025 (30) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Ireland & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1927 - 2025 (99)\\
Israel & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Italy & 1980 - 2025 (46) & 1970 - 2025 (56) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Japan & 1980 - 2025 (46) & 1955 - 2025 (71) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Kazakhstan & 1990 - 2025 (36) & 1990 - 2025 (36) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Kuwait & 2002 - 2025 (24) & 2002 - 2025 (24) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Kyrgyzstan & 1990 - 2025 (36) & 1990 - 2025 (36) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Latvia & 1994 - 2025 (32) & 1994 - 2025 (32) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Lithuania & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Luxembourg & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1960 - 2025 (66)\\
Malaysia & 2006 - 2025 (20) & 2006 - 2025 (20) & 1980 - 2025 (46) & 1948 - 2025 (78)\\
Malta & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Mauritius & 2013 - 2025 (13) & 2013 - 2025 (13) & 1980 - 2025 (46) & 1933 - 2025 (93)\\
Mexico & 1993 - 2025 (33) & 1993 - 2025 (33) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Moldova & 1989 - 2025 (37) & 1989 - 2025 (37) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Mongolia & 2005 - 2025 (21) & 2005 - 2025 (21) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Morocco & 1998 - 2025 (28) & 1998 - 2025 (28) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Netherlands & 1980 - 2025 (46) & 1980 - 2025 (46) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
New Zealand & 1986 - 2025 (40) & 1986 - 2025 (40) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Nicaragua & 2006 - 2025 (20) & 2006 - 2025 (20) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Niger & 1995 - 2025 (31) & 1995 - 2025 (31) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Norway & 1978 - 2025 (48) & 1978 - 2025 (48) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Peru & 2007 - 2025 (19) & 2007 - 2025 (19) & 1980 - 2025 (46) & 1896 - 2025 (130)\\
Philippines & 1993 - 2025 (33) & 1993 - 2025 (33) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Poland & 1991 - 2025 (35) & 1991 - 2025 (35) & 1980 - 2025 (46) & 1924 - 2025 (102)\\
Portugal & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1936 - 2025 (90)\\
Qatar & 2001 - 2025 (25) & 2001 - 2025 (25) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Romania & 1989 - 2025 (37) & 1989 - 2025 (37) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Russia & 1995 - 2025 (31) & 1995 - 2025 (31) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Saudi Arabia & 2002 - 2025 (24) & 2002 - 2025 (24) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Senegal & 2014 - 2025 (12) & 2014 - 2025 (12) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Serbia & 1997 - 2025 (29) & 1997 - 2025 (29) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Slovakia & 1992 - 2025 (34) & 1992 - 2025 (34) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Slovenia & 1995 - 2025 (31) & 1995 - 2025 (31) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
South Africa & 1995 - 2025 (31) & 1995 - 2025 (31) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
South Korea & 1970 - 2025 (56) & 1970 - 2025 (56) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Spain & 1995 - 2025 (31) & 1970 - 2025 (56) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Sweden & 1950 - 2025 (76) & 1810 - 2025 (216) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Switzerland & 1990 - 2025 (36) & 1990 - 2025 (36) & 1980 - 2025 (46) & 1933 - 2025 (93)\\
Trinidad \& Tobago & 1999 - 2025 (27) & 1999 - 2025 (27) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Tunisia & 1992 - 2025 (34) & 1992 - 2025 (34) & 1980 - 2025 (46) & 1946 - 2025 (80)\\
Turkey & 2009 - 2025 (17) & 2009 - 2025 (17) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
USA & 1970 - 2025 (56) & 1970 - 2025 (56) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Ukraine & 1989 - 2025 (37) & 1989 - 2025 (37) & 1980 - 2025 (46) & 1965 - 2025 (61)\\
United Kingdom & 1970 - 2025 (56) & 1920 - 2025 (106) & 1800 - 2025 (226) & 1800 - 2025 (226)\\
Uruguay & 2016 - 2025 (10) & 2016 - 2025 (10) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
Uzbekistan & 2010 - 2025 (16) & 2010 - 2025 (16) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Vanuatu & 2001 - 2025 (25) & 2001 - 2025 (25) & 1980 - 2025 (46) & 1970 - 2025 (56)\\
Venezuela & 1997 - 2025 (29) & 1997 - 2025 (29) & 1980 - 2025 (46) & 1950 - 2025 (76)\\
\bottomrule
\end{tabularx}
\hrule
\end{table}

==> tables/tbl-indicator_table.tex <==
\begin{table}[H]
\caption{Country-level summary of $\theta_s^*$ in the current draft sample. Screen = 0.01. Period reports unscreened country coverage in the analysis file; number of years clearing screen shown in ()}%
\hrule
\makebox[\textwidth][c]{%
{\centering

\begin{tabular}{llrr}
Armenia & 1992 - 2022 (31) & -0.02\\
Aruba & 1997 - 2022 (23) & 0.06\\
Australia & 1961 - 2022 (50) & 0.05\\
Austria & 1997 - 2022 (21) & 0.05\\
Azerbaijan & 1992 - 2022 (28) & 0.12\\
\addlinespace
Bahrain & 2010 - 2022 (13) & 0.07\\
Belarus & 1992 - 2022 (29) & 0.07\\
Belgium & 1987 - 2022 (29) & 0.06\\
Bolivia & 1999 - 2022 (23) & -0.03\\
Botswana & 1991 - 2022 (30) & 0.06\\
\addlinespace
Brazil & 1997 - 2022 (18) & 0.11\\
British Virgin Islands & 1997 - 2022 (23) & 0.05\\
Bulgaria & 1997 - 2022 (19) & 0.13\\
Burkina Faso & 2001 - 2022 (21) & 0.01\\
Cameroon & 1995 - 2022 (26) & 0.02\\
\addlinespace
Canada & 1963 - 2022 (43) & 0.11\\
Cape Verde & 2009 - 2022 (11) & 0.03\\
Chile & 1998 - 2022 (19) & 0.01\\
China & 1994 - 2022 (23) & 0.09\\
Colombia & 1996 - 2022 (24) & 0.05\\
\addlinespace
Costa Rica & 2014 - 2022 (7) & 0.00\\
Croatia & 1997 - 2022 (21) & 0.02\\
Curaçao & 2002 - 2022 (20) & 0.04\\
Cyprus & 1997 - 2022 (24) & 0.11\\
Czechia & 1992 - 2022 (22) & 0.02\\
\addlinespace
Côte d’Ivoire & 1991 - 2022 (27) & 0.06\\
Denmark & 1983 - 2022 (38) & 0.04\\
Dominican Republic & 1993 - 2022 (27) & 0.06\\
Ecuador & 2009 - 2022 (10) & 0.06\\
Egypt & 1998 - 2022 (21) & 0.06\\
\addlinespace
El Salvador & 2016 - 2022 (6) & -0.44\\
Estonia & 1996 - 2022 (23) & -0.06\\
Finland & 1982 - 2022 (29) & -0.01\\
France & 1872 - 2022 (88) & 0.09\\
Germany & 1872 - 2022 (86) & 0.05\\
\addlinespace
Greece & 1997 - 2022 (24) & 0.13\\
Guatemala & 2003 - 2022 (16) & 0.03\\
Guinea & 2005 - 2022 (16) & 0.08\\
Honduras & 2002 - 2022 (15) & 0.11\\
Hong Kong & 1982 - 2022 (37) & 0.08\\
\addlinespace
Hungary & 1997 - 2022 (20) & 0.11\\
Iceland & 2002 - 2022 (17) & 0.06\\
India & 2001 - 2022 (15) & 0.19\\
Indonesia & 2018 - 2022 (5) & 0.01\\
Iran & 1998 - 2022 (24) & 0.04\\
\addlinespace
Ireland & 1997 - 2022 (22) & 0.07\\
Israel & 1997 - 2022 (21) & 0.04\\
\end{tabular}
}

{\centering
\begin{tabular}{llrr}
Italy & 1982 - 2022 (19) & 0.05\\
Japan & 1982 - 2022 (26) & 0.04\\
Kazakhstan & 1992 - 2022 (28) & 0.02\\
Kuwait & 2004 - 2022 (17) & 0.24\\
Kyrgyzstan & 1992 - 2022 (30) & -0.07\\
\addlinespace
Latvia & 1996 - 2022 (26) & 0.00\\
Lithuania & 1997 - 2022 (20) & 0.00\\
Luxembourg & 1997 - 2022 (22) & 0.02\\
Malaysia & 2008 - 2022 (11) & 0.23\\
Malta & 1997 - 2022 (22) & 0.06\\
\addlinespace
Mauritius & 2015 - 2022 (8) & -0.01\\
Mexico & 1995 - 2022 (21) & 0.09\\
Moldova & 1991 - 2022 (32) & -0.04\\
Mongolia & 2007 - 2022 (15) & 0.18\\
Morocco & 2000 - 2022 (18) & 0.01\\
\addlinespace
Netherlands & 1982 - 2022 (28) & -0.01\\
New Zealand & 1988 - 2022 (33) & -0.04\\
Nicaragua & 2008 - 2022 (14) & 0.14\\
Niger & 1997 - 2022 (23) & 0.02\\
Norway & 1980 - 2022 (38) & -0.05\\
\addlinespace
Peru & 2009 - 2022 (12) & 0.06\\
Philippines & 1995 - 2022 (22) & 0.01\\
Poland & 1993 - 2022 (21) & 0.10\\
Portugal & 1997 - 2022 (19) & 0.03\\
Qatar & 2003 - 2022 (19) & 0.21\\
\addlinespace
Romania & 1991 - 2022 (27) & 0.01\\
Russia & 1997 - 2022 (24) & 0.11\\
Saudi Arabia & 2004 - 2022 (14) & 0.12\\
Senegal & 2016 - 2022 (5) & -0.08\\
Serbia & 1999 - 2022 (20) & -0.07\\
\addlinespace
Slovakia & 1994 - 2022 (26) & 0.05\\
Slovenia & 1997 - 2022 (18) & 0.10\\
South Africa & 1997 - 2022 (23) & 0.03\\
South Korea & 1972 - 2022 (41) & 0.00\\
Spain & 1997 - 2022 (21) & 0.07\\
\addlinespace
Sweden & 1952 - 2022 (56) & 0.04\\
Switzerland & 1992 - 2022 (22) & 0.09\\
Trinidad \& Tobago & 2001 - 2022 (20) & 0.00\\
Tunisia & 1994 - 2022 (25) & 0.06\\
Turkey & 2011 - 2022 (11) & 0.02\\
\addlinespace
USA & 1872 - 2022 (89) & -0.03\\
Ukraine & 1991 - 2022 (28) & 0.09\\
United Kingdom & 1857 - 2022 (97) & 0.02\\
Uruguay & 2018 - 2022 (5) & 0.06\\
Uzbekistan & 2012 - 2022 (9) & 0.13\\
\addlinespace
Vanuatu & 2003 - 2022 (15) & 0.03\\
Venezuela & 1999 - 2022 (22) & 0.13\\
\end{tabular}

}

}
\hrule
\label{tbl-indicator_table}
\begin{flushleft}
\footnotesize \emph{Note:} This table is based on observations with $|\Delta g(K)| > 0.01$ in the current analysis file.

\end{flushleft}
\end{table}

==> tables/tbl-pz_wid_comparison_1960_2010.tex <==
\clearpage
\begin{landscape}
\footnotesize
\setlength{\tabcolsep}{1.1pt}
\begin{longtable}{r!{\vrule width 0.9pt}rrrrrr!{\vrule width 0.9pt}rrrrrr!{\vrule width 0.9pt}rrrrrr!{\vrule width 0.9pt}rrrrrr}
\caption{Piketty-Zucman and WID comparison, 1960--2010, in 2010 billions of national currency. PZ levels are computed from PZ 2010-value net national income multiplied by the reported savings share, consumption share, and capital-income ratio. WID monetary levels are already in constant local currency at WID reference-year prices; for this table only, they are converted to 2010 prices using WID's national-income price index before division by $10^9$.}\label{tbl-pz-wid-comparison-1960-2010}\\
\toprule
Year & \multicolumn{6}{c}{France} & \multicolumn{6}{c}{Germany} & \multicolumn{6}{c}{U.K.} & \multicolumn{6}{c}{U.S.}\\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}\cmidrule(lr){14-19}\cmidrule(lr){20-25}
 & \multicolumn{2}{c}{$S_{net}$} & \multicolumn{2}{c}{$C$} & \multicolumn{2}{c}{$K$} & \multicolumn{2}{c}{$S_{net}$} & \multicolumn{2}{c}{$C$} & \multicolumn{2}{c}{$K$} & \multicolumn{2}{c}{$S_{net}$} & \multicolumn{2}{c}{$C$} & \multicolumn{2}{c}{$K$} & \multicolumn{2}{c}{$S_{net}$} & \multicolumn{2}{c}{$C$} & \multicolumn{2}{c}{$K$}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}\cmidrule(lr){20-21}\cmidrule(lr){22-23}\cmidrule(lr){24-25}
 & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID}\\
\midrule
\endfirsthead
\caption[]{Piketty-Zucman and WID comparison, 1960--2010 (continued).}\\
\toprule
Year & \multicolumn{6}{c}{France} & \multicolumn{6}{c}{Germany} & \multicolumn{6}{c}{U.K.} & \multicolumn{6}{c}{U.S.}\\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}\cmidrule(lr){14-19}\cmidrule(lr){20-25}
 & \multicolumn{2}{c}{$S_{net}$} & \multicolumn{2}{c}{$C$} & \multicolumn{2}{c}{$K$} & \multicolumn{2}{c}{$S_{net}$} & \multicolumn{2}{c}{$C$} & \multicolumn{2}{c}{$K$} & \multicolumn{2}{c}{$S_{net}$} & \multicolumn{2}{c}{$C$} & \multicolumn{2}{c}{$K$} & \multicolumn{2}{c}{$S_{net}$} & \multicolumn{2}{c}{$C$} & \multicolumn{2}{c}{$K$}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}\cmidrule(lr){20-21}\cmidrule(lr){22-23}\cmidrule(lr){24-25}
 & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID} & \multicolumn{1}{c}{PZ} & \multicolumn{1}{c}{WID}\\
\midrule
\endhead
\midrule
\multicolumn{25}{r}{Continued on next page}\\
\endfoot
\bottomrule
\endlastfoot
1960 & 73 & 68 & 334 & 329 & 1378 & 1314 & 141 & 145 & 461 &  & 1535 & 1500 & 42 & 59 & 378 &  & 1104 & 1300 & 326 &  & 2475 &  & 11595 & 9139\\
1961 & 72 & 67 & 354 & 349 & 1481 & 1408 & 139 & 146 & 485 &  & 1700 & 1718 & 47 & 51 & 389 &  & 1186 & 1372 & 331 &  & 2538 &  & 12216 & 10718\\
1962 & 78 & 71 & 379 & 373 & 1588 & 1510 & 135 & 143 & 514 &  & 1846 & 1942 & 43 & 49 & 395 &  & 1217 & 1440 & 374 &  & 2677 &  & 12791 & 11232\\
1963 & 81 & 74 & 405 & 398 & 1707 & 1623 & 130 & 137 & 534 &  & 1987 & 2110 & 45 & 43 & 404 &  & 1336 & 1618 & 402 &  & 2794 &  & 13238 & 11561\\
1964 & 91 & 84 & 426 & 419 & 1829 & 1740 & 152 & 162 & 555 &  & 2126 & 2260 & 56 & 54 & 419 &  & 1382 & 1665 & 437 &  & 2948 &  & 13927 & 12129\\
1965 & 98 & 91 & 443 & 435 & 1963 & 1868 & 150 & 159 & 592 &  & 2233 & 2382 & 58 & 55 & 427 &  & 1381 & 1693 & 488 &  & 3116 &  & 14801 & 12889\\
1966 & 103 & 96 & 465 & 458 & 2111 & 2009 & 147 & 156 & 612 &  & 2344 & 2526 & 58 & 54 & 433 &  & 1438 & 1744 & 500 &  & 3317 &  & 15251 & 13251\\
1967 & 107 & 98 & 489 & 481 & 2261 & 2151 & 128 & 136 & 624 &  & 2506 & 2711 & 57 & 51 & 445 &  & 1527 & 1847 & 460 &  & 3452 &  & 15897 & 13772\\
1968 & 106 & 96 & 515 & 507 & 2418 & 2295 & 151 & 162 & 644 &  & 2661 & 2844 & 63 & 59 & 459 &  & 1592 & 1931 & 462 &  & 3646 &  & 17000 & 14746\\
1969 & 116 & 106 & 549 & 541 & 2590 & 2458 & 174 & 190 & 685 &  & 2812 & 3002 & 71 & 77 & 466 &  & 1633 & 2007 & 476 &  & 3761 &  & 17269 & 14951\\
1970 & 126 & 116 & 577 & 570 & 2502 & 2304 & 188 & 216 & 713 & 817 & 2865 & 3203 & 72 & 78 & 477 & 518 & 1729 & 2125 & 385 & 438 & 3824 & 3744 & 17105 & 14670\\
1971 & 132 & 120 & 610 & 597 & 2611 & 2401 & 176 & 203 & 748 & 853 & 2894 & 3340 & 70 & 65 & 483 & 547 & 1898 & 2258 & 397 & 448 & 3936 & 3872 & 17669 & 15122\\
1972 & 139 & 127 & 637 & 621 & 2770 & 2546 & 170 & 196 & 791 & 904 & 3023 & 3563 & 56 & 62 & 515 & 574 & 2138 & 2471 & 458 & 513 & 4126 & 4046 & 19059 & 16326\\
1973 & 152 & 138 & 674 & 657 & 2942 & 2688 & 176 & 203 & 831 & 951 & 3130 & 3770 & 68 & 64 & 545 & 616 & 2261 & 2704 & 597 & 638 & 4287 & 4197 & 19889 & 17052\\
1974 & 149 & 135 & 713 & 691 & 3068 & 2808 & 158 & 182 & 852 & 975 & 3178 & 3956 & 44 & 11 & 547 & 644 & 2194 & 2799 & 500 & 534 & 4320 & 4235 & 19208 & 16411\\
1975 & 118 & 105 & 726 & 715 & 3162 & 2907 & 113 & 130 & 884 & 1014 & 3213 & 4055 & 35 & 2 & 546 & 633 & 1929 & 2497 & 352 & 386 & 4389 & 4316 & 18957 & 16164\\
1976 & 117 & 105 & 761 & 750 & 3285 & 3027 & 129 & 149 & 921 & 1056 & 3298 & 4142 & 50 & 7 & 544 & 647 & 1853 & 2379 & 418 & 453 & 4587 & 4520 & 20012 & 17097\\
1977 & 118 & 107 & 788 & 776 & 3414 & 3144 & 130 & 150 & 954 & 1089 & 3457 & 4259 & 52 & 24 & 554 & 637 & 1870 & 2377 & 484 & 514 & 4772 & 4690 & 20790 & 17801\\
1978 & 115 & 101 & 821 & 817 & 3538 & 3310 & 141 & 163 & 977 & 1117 & 3657 & 4397 & 54 & 31 & 562 & 660 & 1999 & 2537 & 590 & 625 & 4952 & 4869 & 21629 & 18535\\
1979 & 120 & 104 & 851 & 848 & 3691 & 3490 & 138 & 159 & 1021 & 1172 & 3819 & 4552 & 49 & 30 & 582 & 688 & 2179 & 2787 & 594 & 632 & 5077 & 5030 & 22972 & 19744\\
1980 & 109 & 97 & 878 & 865 & 3819 & 3623 & 115 & 128 & 1051 & 1188 & 3916 & 5343 & 34 & 21 & 582 & 674 & 2132 & 2849 & 461 & 488 & 5160 & 5100 & 24512 & 21281\\
1981 & 78 & 64 & 913 & 903 & 3854 & 3685 & 94 & 102 & 1072 & 1212 & 4014 & 5560 & 27 & 23 & 580 & 668 & 2124 & 2892 & 536 & 568 & 5224 & 5149 & 24920 & 21858\\
1982 & 64 & 49 & 944 & 936 & 3817 & 3668 & 94 & 101 & 1062 & 1201 & 4072 & 5751 & 27 & 33 & 599 & 676 & 2194 & 2894 & 376 & 406 & 5291 & 5152 & 24962 & 22157\\
1983 & 59 & 46 & 954 & 944 & 3844 & 3692 & 101 & 111 & 1077 & 1215 & 4188 & 5936 & 33 & 30 & 622 & 714 & 2310 & 3051 & 291 & 331 & 5581 & 5505 & 25326 & 22615\\
1984 & 58 & 40 & 971 & 963 & 3884 & 3728 & 111 & 123 & 1102 & 1244 & 4339 & 6240 & 36 & 37 & 639 & 728 & 2460 & 3251 & 518 & 564 & 5861 & 5744 & 25695 & 23253\\
1985 & 57 & 36 & 994 & 990 & 3912 & 3755 & 125 & 139 & 1117 & 1262 & 4503 & 6491 & 40 & 43 & 656 & 751 & 2602 & 3394 & 419 & 478 & 6191 & 6073 & 26681 & 24451\\
1986 & 77 & 60 & 1005 & 991 & 4006 & 3839 & 153 & 170 & 1120 & 1261 & 4635 & 6637 & 33 & 31 & 697 & 794 & 2891 & 3672 & 301 & 362 & 6472 & 6383 & 28281 & 26239\\
1987 & 74 & 61 & 1036 & 1017 & 4171 & 3978 & 142 & 157 & 1145 & 1290 & 4809 & 6912 & 37 & 97 & 721 & 765 & 3212 & 3830 & 361 & 416 & 6699 & 6562 & 29346 & 27436\\
1988 & 98 & 82 & 1064 & 1050 & 4344 & 4123 & 167 & 186 & 1176 & 1326 & 4976 & 7174 & 41 & 107 & 757 & 809 & 3681 & 4158 & 481 & 523 & 6958 & 6768 & 30282 & 28387\\
1989 & 114 & 99 & 1097 & 1083 & 4665 & 4392 & 190 & 215 & 1208 & 1362 & 5139 & 7601 & 43 & 112 & 771 & 826 & 4077 & 4519 & 434 & 473 & 7174 & 7080 & 31602 & 29635\\
1990 & 113 & 95 & 1126 & 1116 & 4842 & 4547 & 193 & 225 & 1253 & 1440 & 5342 & 7525 & 33 & 97 & 782 & 842 & 4020 & 4438 & 336 & 387 & 7375 & 7310 & 31871 & 29854\\
1991 & 105 & 84 & 1142 & 1129 & 4833 & 4545 & 172 & 173 & 1495 & 1569 & 5870 & 7923 & 19 & 84 & 785 & 840 & 3819 & 4281 & 329 & 316 & 7411 & 7356 & 31896 & 29895\\
1992 & 103 & 79 & 1168 & 1154 & 4825 & 4532 & 168 & 169 & 1535 & 1600 & 5925 & 8606 & 11 & 72 & 798 & 865 & 3714 & 4239 & 274 & 334 & 7661 & 7641 & 32553 & 30331\\
1993 & 82 & 60 & 1180 & 1160 & 4796 & 4489 & 136 & 131 & 1535 & 1605 & 5985 & 8187 & 12 & 75 & 817 & 888 & 3763 & 4379 & 255 & 293 & 7881 & 7903 & 33080 & 30678\\
1994 & 86 & 65 & 1198 & 1189 & 4785 & 4475 & 136 & 132 & 1563 & 1639 & 6096 & 8168 & 32 & 94 & 841 & 914 & 3838 & 4414 & 381 & 400 & 8136 & 8130 & 33639 & 31352\\
1995 & 102 & 77 & 1217 & 1206 & 4740 & 4565 & 141 & 103 & 1587 & 1692 & 6106 & 7915 & 40 & 70 & 859 & 954 & 3838 & 3823 & 475 & 477 & 8336 & 8274 & 35235 & 32885\\
1996 & 97 & 75 & 1242 & 1232 & 4765 & 4787 & 129 & 117 & 1614 & 1692 & 6200 & 7225 & 46 & 76 & 884 & 975 & 3982 & 3835 & 576 & 605 & 8609 & 8496 & 37837 & 35516\\
1997 & 123 & 101 & 1252 & 1254 & 4907 & 4899 & 136 & 123 & 1634 & 1712 & 6423 & 7470 & 64 & 42 & 906 & 1055 & 4332 & 4121 & 736 & 776 & 8909 & 8737 & 41188 & 39122\\
1998 & 148 & 124 & 1279 & 1285 & 5081 & 5080 & 144 & 136 & 1651 & 1729 & 6633 & 7690 & 78 & 54 & 943 & 1095 & 4768 & 4536 & 822 & 878 & 9314 & 9058 & 46048 & 43986\\
1999 & 164 & 145 & 1317 & 1324 & 5609 & 5578 & 132 & 126 & 1694 & 1769 & 6889 & 8132 & 53 & 31 & 988 & 1132 & 5293 & 5002 & 779 & 852 & 9824 & 9555 & 51702 & 48941\\
2000 & 166 & 147 & 1366 & 1370 & 6124 & 6061 & 129 & 124 & 1747 & 1823 & 7216 & 8621 & 47 & 44 & 1042 & 1180 & 5823 & 5384 & 770 & 845 & 10329 & 9973 & 54530 & 51456\\
2001 & 158 & 141 & 1395 & 1406 & 6343 & 6233 & 123 & 118 & 1780 & 1857 & 7329 & 8628 & 54 & 37 & 1084 & 1221 & 5900 & 5551 & 553 & 664 & 10610 & 10222 & 53888 & 51528\\
2002 & 131 & 109 & 1418 & 1438 & 6548 & 6395 & 120 & 112 & 1775 & 1847 & 7308 & 8457 & 54 & 30 & 1121 & 1256 & 5818 & 5714 & 307 & 499 & 10930 & 10550 & 52440 & 50624\\
2003 & 112 & 97 & 1444 & 1465 & 7015 & 6882 & 113 & 97 & 1786 & 1847 & 7381 & 8298 & 58 & 47 & 1162 & 1284 & 6017 & 6038 & 232 & 414 & 11273 & 10966 & 54137 & 52134\\
2004 & 130 & 111 & 1476 & 1495 & 7805 & 7690 & 175 & 158 & 1786 & 1849 & 7567 & 8319 & 55 & 45 & 1197 & 1313 & 6396 & 6447 & 337 & 502 & 11635 & 11345 & 59519 & 57404\\
2005 & 124 & 107 & 1508 & 1528 & 8769 & 8629 & 176 & 156 & 1803 & 1869 & 7780 & 8483 & 51 & 57 & 1233 & 1346 & 6809 & 6823 & 416 & 557 & 11984 & 11669 & 64813 & 62338\\
2006 & 140 & 121 & 1536 & 1555 & 9741 & 9577 & 244 & 222 & 1839 & 1909 & 8022 & 8691 & 48 & 48 & 1253 & 1357 & 7168 & 7128 & 550 & 668 & 12274 & 11847 & 69706 & 66674\\
2007 & 152 & 130 & 1560 & 1584 & 10435 & 10209 & 306 & 285 & 1837 & 1902 & 8359 & 8974 & 76 & 52 & 1284 & 1391 & 7535 & 7401 & 257 & 410 & 12563 & 12341 & 70963 & 68411\\
2008 & 130 & 105 & 1570 & 1605 & 10298 & 9893 & 271 & 239 & 1873 & 1947 & 8660 & 9205 & 79 & 25 & 1285 & 1409 & 7058 & 6860 & -60 & -3 & 12764 & 12745 & 62219 & 61042\\
2009 & 60 & 46 & 1575 & 1602 & 9981 & 9494 & 157 & 137 & 1874 & 1929 & 8706 & 9138 & 22 & -26 & 1255 & 1389 & 6675 & 6473 & -332 & -228 & 12556 & 12591 & 54609 & 53219\\
2010 & 65 & 51 & 1604 & 1633 & 10302 & 9786 & 196 & 187 & 1912 & 1972 & 8919 & 9312 & 27 & 7 & 1271 & 1404 & 6857 & 6671 & -172 & 40 & 12840 & 12789 & 55230 & 53421\\
\end{longtable}
\normalsize
\end{landscape}
\clearpage


==> tables/tbl-pz_wid_overlap_percent_differences.tex <==
\begin{table}[H]
\caption{Mean signed percent differences between WID and Piketty-Zucman by available overlap decade, with a total row. Percent difference is $100\times(WID-PZ)/|PZ|$, after converting WID monetary levels to 2010 prices using WID's national-income price index.}\label{tbl-pz-wid-overlap-percent-differences}
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l!{\vrule width 0.9pt}rrr!{\vrule width 0.9pt}rrr!{\vrule width 0.9pt}rrr!{\vrule width 0.9pt}rrr}
\toprule
Period & \multicolumn{3}{c}{France} & \multicolumn{3}{c}{Germany} & \multicolumn{3}{c}{U.K.} & \multicolumn{3}{c}{U.S.}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
 & $S_{net}$ & $C$ & $K$ & $S_{net}$ & $C$ & $K$ & $S_{net}$ & $C$ & $K$ & $S_{net}$ & $C$ & $K$\\
\midrule
1870s &  &  & -24.3 &  &  & -45.8 &  &  & +26.5 &  &  & +31.2\\
1880s &  &  & -24.2 &  &  & -39.3 &  &  & +22.7 &  &  & +39.4\\
1890s & -19.3 &  & -21.5 &  &  & -42.5 &  &  & +10.9 &  &  & +32.9\\
1900s & -15.1 &  & -13.2 &  &  & -52.7 &  &  & +9.0 &  &  & +46.8\\
1910s & +1.0 &  & -15.1 &  &  & -51.0 &  &  & +4.7 &  &  & +35.4\\
1920s & -3.9 &  & -7.0 &  &  & -40.9 & -108.8 &  & +14.2 &  &  & +19.1\\
1930s & -3.4 &  & -4.6 &  &  & -45.5 & -86.2 &  & +11.8 &  &  & +3.8\\
1940s & -3.8 &  & -8.4 &  &  & -51.5 & -250.3 &  & +21.8 &  &  & -16.0\\
1950s & -14.4 & -4.2 & -7.0 & +0.6 &  & -11.5 & +22.1 &  & +25.6 &  &  & -31.2\\
1960s & -7.9 & -1.6 & -4.9 & +6.2 &  & +5.3 & +3.5 &  & +20.2 &  &  & -13.7\\
1970s & -10.0 & -1.7 & -7.7 & +15.2 & +14.5 & +20.5 & -38.2 & +15.0 & +24.4 & +8.9 & -1.7 & -14.4\\
1980s & -21.3 & -1.1 & -4.5 & +10.5 & +12.9 & +42.5 & +44.8 & +12.1 & +26.6 & +11.0 & -1.8 & -9.1\\
1990s & -20.5 & -0.6 & -3.5 & -4.5 & +5.9 & +28.8 & +187.1 & +10.9 & +4.9 & +8.0 & -1.1 & -6.1\\
2000s & -15.1 & +1.3 & -2.3 & -9.0 & +3.8 & +11.1 & -42.4 & +10.4 & -2.2 & +46.1 & -2.4 & -3.7\\
2010s & -21.0 & +1.8 & -5.0 & -4.6 & +3.1 & +4.4 & -73.9 & +10.5 & -2.7 & +123.1 & -0.4 & -3.3\\
Total & -10.8 & -1.3 & -10.5 & +3.1 & +9.1 & -19.3 & -12.8 & +12.1 & +15.7 & +21.1 & -1.7 & +8.1\\
\bottomrule
\end{tabular}
\normalsize
\end{table}


==> tables/tbl-reg_s.tex <==
\centering
\begin{tabularx}{\columnwidth}{lcc}
   \midrule 
   Regression of $s^*$ on \(g(K)\)             & 0.0771$^{***}$ &   \\   
   Regression of value shown on $\Delta g(K)$  &                & 0.0559$^{***}$\\   
                                               &                & (0.0057)\\   
    \\
   Observations                                & 1,826          & 1,574\\  
   R$^2$                                       & 0.84511        & 0.37071\\  
   Within R$^2$                                & 0.10669        & 0.27233\\  
    \\
   Year fixed effects                          & $\checkmark$   & $\checkmark$\\   
   Country fixed effects                       & $\checkmark$   & $\checkmark$\\   
   \bottomrule
\end{tabularx}
   \label{tbl-reg_s}


==> tables/tbl-thrift_predictions.tex <==
\begingroup
\tiny
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}
\begin{longtable}{lcccccccc}
\caption{Regressions of $s^*$ on $g(K)$ and $\Delta s^*$ on $\Delta g(K)$ by country. Screen = 0.01 for the differenced regressions. $H_0$ per thrift theory: all regressions $\cong 1$.}\label{tab:thrift_predictions}\\
\toprule
 & \multicolumn{4}{c}{$s^*$ on $g(K)$} & \multicolumn{4}{c}{$\Delta s^*$ on $\Delta g(K)$}\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
Country & Coef. & S.E. & Obs. & R$^2$ & Coef. & S.E. & Obs. & R$^2$\\
\midrule
\endfirsthead
\toprule
 & \multicolumn{4}{c}{$s^*$ on $g(K)$} & \multicolumn{4}{c}{$\Delta s^*$ on $\Delta g(K)$}\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
Country & Coef. & S.E. & Obs. & R$^2$ & Coef. & S.E. & Obs. & R$^2$\\
\midrule
\endhead
Armenia & 0.008 & (0.053) & 29 & 0.001 & -0.005 & (0.023) & 31 & 0.002\\
Aruba & 0.029$^{**}$ & (0.010) & 25 & 0.161 & 0.022$^{***}$ & (0.004) & 23 & 0.375\\
Australia & 0.066 & (0.044) & 54 & 0.029 & 0.023$^{*}$ & (0.011) & 50 & 0.099\\
Austria & 0.051$^{**}$ & (0.024) & 23 & 0.167 & 0.041$^{*}$ & (0.020) & 21 & 0.218\\
Azerbaijan & 0.220$^{***}$ & (0.043) & 30 & 0.366 & 0.025 & (0.042) & 28 & 0.019\\
Bahrain & 0.087$^{***}$ & (0.022) & 12 & 0.499 & 0.096$^{**}$ & (0.031) & 13 & 0.724\\
Belarus & 0.013 & (0.031) & 30 & 0.012 & 0.009 & (0.018) & 29 & 0.014\\
Belgium & 0.164$^{***}$ & (0.044) & 29 & 0.197 & 0.064$^{***}$ & (0.019) & 29 & 0.308\\
Bolivia & 0.130$^{***}$ & (0.036) & 23 & 0.240 & 0.015 & (0.029) & 23 & 0.014\\
Botswana & 0.118$^{***}$ & (0.029) & 31 & 0.297 & 0.072$^{***}$ & (0.018) & 30 & 0.331\\
Brazil & 0.160$^{***}$ & (0.033) & 20 & 0.630 & 0.091$^{***}$ & (0.024) & 18 & 0.499\\
British Virgin Islands & 0.029$^{***}$ & (0.006) & 25 & 0.239 & 0.018 & (0.011) & 23 & 0.378\\
Bulgaria & 0.127$^{***}$ & (0.016) & 23 & 0.351 & 0.111 & (0.070) & 19 & 0.358\\
Burkina Faso & -0.067 & (0.045) & 21 & 0.083 & 0.023 & (0.016) & 21 & 0.073\\
Cameroon & 0.032 & (0.044) & 24 & 0.039 & 0.055$^{**}$ & (0.020) & 26 & 0.321\\
Canada & 0.069 & (0.056) & 53 & 0.019 & 0.012 & (0.022) & 43 & 0.007\\
Cape Verde & 0.018$^{*}$ & (0.010) & 13 & 0.053 & 0.015$^{***}$ & (0.004) & 11 & 0.102\\
Chile & 0.091 & (0.096) & 23 & 0.093 & 0.024 & (0.020) & 19 & 0.047\\
China & 0.117$^{**}$ & (0.052) & 30 & 0.135 & 0.054$^{***}$ & (0.013) & 23 & 0.359\\
Colombia & 0.043 & (0.061) & 27 & 0.047 & 0.020 & (0.022) & 24 & 0.057\\
Costa Rica & -0.000 & (0.007) & 8 & 0.000 & 0.014 & (0.014) & 7 & 0.220\\
Croatia & 0.047$^{**}$ & (0.017) & 23 & 0.113 & 0.009 & (0.018) & 21 & 0.015\\
Curaçao & 0.056 & (0.058) & 20 & 0.033 & 0.014 & (0.031) & 20 & 0.020\\
Cyprus & 0.039 & (0.033) & 22 & 0.053 & 0.007 & (0.044) & 24 & 0.003\\
Czechia & 0.028$^{*}$ & (0.014) & 26 & 0.085 & 0.048$^{**}$ & (0.018) & 22 & 0.241\\
Côte d’Ivoire & 0.154$^{**}$ & (0.063) & 32 & 0.202 & 0.022 & (0.027) & 27 & 0.021\\
Denmark & 0.050$^{**}$ & (0.019) & 40 & 0.238 & 0.024$^{**}$ & (0.010) & 38 & 0.160\\
Dominican Republic & 0.048$^{*}$ & (0.027) & 28 & 0.110 & 0.038$^{***}$ & (0.011) & 27 & 0.226\\
Ecuador & 0.053$^{***}$ & (0.011) & 15 & 0.511 & 0.035$^{***}$ & (0.004) & 10 & 0.721\\
Egypt & 0.051 & (0.033) & 22 & 0.044 & 0.021$^{***}$ & (0.007) & 21 & 0.156\\
El Salvador & -0.090 & (0.183) & 7 & 0.058 & -0.028 & (0.025) & 6 & 0.049\\
Estonia & 0.133$^{***}$ & (0.023) & 27 & 0.570 & 0.061$^{*}$ & (0.033) & 23 & 0.151\\
Finland & 0.149$^{**}$ & (0.059) & 36 & 0.281 & 0.022 & (0.018) & 29 & 0.047\\
France & 0.173$^{***}$ & (0.031) & 124 & 0.302 & 0.035$^{**}$ & (0.017) & 88 & 0.091\\
Germany & 0.296$^{***}$ & (0.072) & 119 & 0.329 & 0.056$^{***}$ & (0.009) & 86 & 0.269\\
Greece & 0.134$^{***}$ & (0.026) & 24 & 0.541 & 0.070$^{***}$ & (0.020) & 24 & 0.438\\
Guatemala & -0.036 & (0.084) & 19 & 0.029 & 0.004 & (0.040) & 16 & 0.002\\
Guinea & 0.032$^{***}$ & (0.010) & 19 & 0.142 & 0.042$^{***}$ & (0.009) & 16 & 0.327\\
Honduras & 0.019 & (0.054) & 16 & 0.008 & 0.020 & (0.020) & 15 & 0.041\\
Hong Kong & 0.191$^{***}$ & (0.045) & 41 & 0.307 & 0.051$^{**}$ & (0.021) & 37 & 0.199\\
Hungary & 0.196$^{***}$ & (0.039) & 23 & 0.447 & 0.069$^{**}$ & (0.027) & 20 & 0.288\\
Iceland & 0.138$^{***}$ & (0.032) & 19 & 0.510 & 0.084$^{***}$ & (0.022) & 17 & 0.501\\
India & 0.087 & (0.075) & 23 & 0.176 & 0.025$^{*}$ & (0.012) & 15 & 0.118\\
Indonesia & 0.021 & (0.026) & 5 & 0.068 & 0.003 & (0.019) & 5 & 0.011\\
Iran & 0.188$^{***}$ & (0.048) & 20 & 0.371 & 0.097$^{***}$ & (0.033) & 24 & 0.308\\
Ireland & 0.112$^{***}$ & (0.021) & 25 & 0.537 & 0.073$^{***}$ & (0.022) & 22 & 0.395\\
Israel & -0.025 & (0.055) & 25 & 0.010 & 0.034 & (0.021) & 21 & 0.145\\
Italy & 0.081$^{***}$ & (0.028) & 35 & 0.177 & 0.015 & (0.014) & 19 & 0.073\\
Japan & 0.116$^{***}$ & (0.026) & 28 & 0.339 & 0.013 & (0.011) & 26 & 0.049\\
Kazakhstan & 0.153$^{***}$ & (0.055) & 29 & 0.306 & 0.046$^{**}$ & (0.019) & 28 & 0.142\\
Kuwait & 0.174$^{*}$ & (0.082) & 18 & 0.199 & 0.048$^{*}$ & (0.026) & 17 & 0.064\\
Kyrgyzstan & -0.043 & (0.033) & 31 & 0.038 & -0.019 & (0.020) & 30 & 0.025\\
Latvia & 0.032 & (0.113) & 26 & 0.005 & -0.056$^{***}$ & (0.020) & 26 & 0.106\\
Lithuania & -0.048 & (0.080) & 25 & 0.028 & 0.019 & (0.045) & 20 & 0.018\\
Luxembourg & 0.010 & (0.035) & 24 & 0.001 & -0.021 & (0.026) & 22 & 0.044\\
Malaysia & 0.232$^{***}$ & (0.074) & 16 & 0.237 & 0.063 & (0.052) & 11 & 0.204\\
Malta & 0.420$^{***}$ & (0.125) & 24 & 0.384 & 0.103 & (0.064) & 22 & 0.098\\
Mauritius & -0.007 & (0.005) & 8 & 0.231 & -0.007$^{***}$ & (0.002) & 8 & 0.613\\
Mexico & 0.063$^{*}$ & (0.033) & 25 & 0.132 & 0.042 & (0.030) & 21 & 0.148\\
Moldova & -0.043 & (0.067) & 31 & 0.042 & 0.035 & (0.021) & 32 & 0.174\\
Mongolia & 0.155$^{***}$ & (0.033) & 15 & 0.723 & 0.108$^{***}$ & (0.015) & 15 & 0.674\\
Morocco & 0.057$^{**}$ & (0.022) & 22 & 0.132 & 0.032$^{***}$ & (0.011) & 18 & 0.251\\
Netherlands & 0.061$^{*}$ & (0.031) & 38 & 0.155 & 0.023 & (0.018) & 28 & 0.036\\
New Zealand & 0.011 & (0.031) & 32 & 0.003 & 0.044 & (0.027) & 33 & 0.051\\
Nicaragua & 0.036 & (0.053) & 14 & 0.041 & 0.023 & (0.018) & 14 & 0.086\\
Niger & 0.032 & (0.030) & 27 & 0.032 & 0.036$^{***}$ & (0.010) & 23 & 0.220\\
Norway & -0.001 & (0.043) & 42 & 0.000 & -0.045$^{**}$ & (0.022) & 38 & 0.086\\
Peru & 0.031 & (0.038) & 15 & 0.086 & 0.022 & (0.021) & 12 & 0.133\\
Philippines & 0.121 & (0.093) & 28 & 0.106 & 0.041 & (0.035) & 22 & 0.076\\
Poland & 0.050 & (0.036) & 30 & 0.068 & 0.066$^{*}$ & (0.033) & 21 & 0.371\\
Portugal & 0.060$^{**}$ & (0.026) & 22 & 0.203 & 0.010 & (0.015) & 19 & 0.023\\
Qatar & 0.294$^{***}$ & (0.041) & 20 & 0.756 & 0.129$^{*}$ & (0.073) & 19 & 0.279\\
Romania & 0.007 & (0.028) & 30 & 0.002 & -0.007 & (0.011) & 27 & 0.018\\
Russia & 0.048$^{*}$ & (0.026) & 22 & 0.123 & 0.027 & (0.024) & 24 & 0.034\\
Saudi Arabia & 0.193$^{***}$ & (0.051) & 17 & 0.373 & 0.092$^{**}$ & (0.037) & 14 & 0.330\\
Senegal & -0.153 & (0.091) & 8 & 0.320 & -0.058$^{*}$ & (0.022) & 5 & 0.396\\
Serbia & -0.137 & (0.086) & 25 & 0.135 & -0.090 & (0.076) & 20 & 0.215\\
Slovakia & 0.148$^{***}$ & (0.050) & 24 & 0.194 & 0.058 & (0.046) & 26 & 0.109\\
Slovenia & 0.166$^{***}$ & (0.035) & 26 & 0.544 & 0.099$^{**}$ & (0.041) & 18 & 0.399\\
South Africa & 0.063 & (0.037) & 18 & 0.186 & 0.039$^{**}$ & (0.017) & 23 & 0.178\\
South Korea & 0.081$^{**}$ & (0.034) & 51 & 0.088 & 0.059$^{***}$ & (0.017) & 41 & 0.390\\
Spain & 0.084$^{***}$ & (0.013) & 22 & 0.563 & 0.028$^{**}$ & (0.012) & 21 & 0.187\\
Sweden & 0.096$^{**}$ & (0.037) & 64 & 0.104 & 0.053$^{***}$ & (0.018) & 56 & 0.162\\
Switzerland & 0.038 & (0.032) & 24 & 0.027 & 0.075$^{*}$ & (0.040) & 22 & 0.149\\
Trinidad \& Tobago & 0.005$^{***}$ & (0.001) & 22 & 0.672 & 0.002$^{***}$ & (0.000) & 20 & 0.624\\
Tunisia & 0.086 & (0.056) & 27 & 0.090 & 0.004 & (0.018) & 25 & 0.002\\
Turkey & -0.045 & (0.153) & 13 & 0.014 & -0.042 & (0.027) & 11 & 0.137\\
USA & 0.032 & (0.027) & 142 & 0.017 & 0.004 & (0.010) & 89 & 0.002\\
Ukraine & 0.012 & (0.022) & 30 & 0.009 & 0.020$^{*}$ & (0.010) & 28 & 0.115\\
United Kingdom & 0.096$^{***}$ & (0.023) & 142 & 0.165 & 0.008 & (0.014) & 97 & 0.006\\
Uruguay & 0.022 & (0.018) & 6 & 0.195 & 0.026 & (0.014) & 5 & 0.448\\
Uzbekistan & 0.163 & (0.123) & 12 & 0.124 & 0.018 & (0.032) & 9 & 0.060\\
Vanuatu & 0.060 & (0.058) & 19 & 0.113 & 0.028$^{**}$ & (0.012) & 15 & 0.258\\
Venezuela & 0.137$^{***}$ & (0.025) & 22 & 0.542 & 0.037 & (0.030) & 22 & 0.126\\
\bottomrule
\end{longtable}
\begin{flushleft}
\footnotesize \emph{Note:} Entries show coefficient estimates and HC1 standard errors in separate columns. Three, two and one asterisks denote $p<0.01$, $p<0.05$ and $p<0.10$, respectively.
\end{flushleft}
\endgroup


==> tables/tbl-wid-pz-year-ranges.tex <==
\begin{table}[H]
\caption{Source coverage in the final analysis sample by country. Year ranges report the observations taken from WID and, where WID is incomplete, from PZ. WID is given priority whenever it reports a complete country-year. Missing entries are shown as --.}\label{tbl-wid-pz-year-ranges}
\scriptsize
\setlength{\tabcolsep}{4pt}
\makebox[\textwidth][c]{%
\begin{minipage}[t]{0.49\textwidth}
\vspace{0pt}
\centering
\begin{tabular}{p{0.34\linewidth}p{0.28\linewidth}p{0.28\linewidth}}
\toprule
Country & WID & PZ\\
\midrule
Armenia & 1990--2022 & --\\
Aruba & 1995--2022 & --\\
Australia & 1959--2022 & --\\
Austria & 1995--2022 & --\\
Azerbaijan & 1990--2022 & --\\
Bahrain & 2008--2022 & --\\
Belarus & 1990--2022 & --\\
Belgium & 1985--2022 & --\\
Bolivia & 1997--2022 & --\\
Botswana & 1989--2022 & --\\
Brazil & 1995--2022 & --\\
British Virgin Islands & 1995--2022 & --\\
Bulgaria & 1995--2022 & --\\
Burkina Faso & 1999--2022 & --\\
Cameroon & 1993--2022 & --\\
Canada & 1961--2022 & --\\
Cape Verde & 2007--2022 & --\\
Chile & 1996--2022 & --\\
China & 1992--2022 & --\\
Colombia & 1994--2022 & --\\
Costa Rica & 2012--2022 & --\\
Croatia & 1995--2022 & --\\
Curaçao & 2000--2022 & --\\
Cyprus & 1995--2022 & --\\
Czechia & 1990--2022 & --\\
Côte d’Ivoire & 1989--2022 & --\\
Denmark & 1981--2022 & --\\
Dominican Republic & 1991--2022 & --\\
Ecuador & 2007--2022 & --\\
Egypt & 1996--2022 & --\\
El Salvador & 2014--2022 & --\\
Estonia & 1994--2022 & --\\
Finland & 1980--2022 & --\\
France & 1950--2022 & 1870--1949\\
Germany & 1970--2022 & 1870--1913, 1925--1938, 1950--1969\\
Greece & 1995--2022 & --\\
Guatemala & 2001--2022 & --\\
Guinea & 2003--2022 & --\\
Honduras & 2000--2022 & --\\
Hong Kong & 1980--2022 & --\\
Hungary & 1995--2022 & --\\
Iceland & 2000--2022 & --\\
India & 1999--2022 & --\\
Indonesia & 2016--2022 & --\\
Iran & 1996--2022 & --\\
Ireland & 1995--2022 & --\\
Israel & 1995--2022 & --\\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\textwidth}
\vspace{0pt}
\centering
\begin{tabular}{p{0.34\linewidth}p{0.28\linewidth}p{0.28\linewidth}}
\toprule
Country & WID & PZ\\
\midrule
Italy & 1980--2022 & --\\
Japan & 1980--2022 & --\\
Kazakhstan & 1990--2022 & --\\
Kuwait & 2002--2022 & --\\
Kyrgyzstan & 1990--2022 & --\\
Latvia & 1994--2022 & --\\
Lithuania & 1995--2022 & --\\
Luxembourg & 1995--2022 & --\\
Malaysia & 2006--2022 & --\\
Malta & 1995--2022 & --\\
Mauritius & 2013--2022 & --\\
Mexico & 1993--2022 & --\\
Moldova & 1989--2022 & --\\
Mongolia & 2005--2022 & --\\
Morocco & 1998--2022 & --\\
Netherlands & 1980--2022 & --\\
New Zealand & 1986--2022 & --\\
Nicaragua & 2006--2022 & --\\
Niger & 1995--2022 & --\\
Norway & 1978--2022 & --\\
Peru & 2007--2022 & --\\
Philippines & 1993--2022 & --\\
Poland & 1991--2022 & --\\
Portugal & 1995--2022 & --\\
Qatar & 2001--2022 & --\\
Romania & 1989--2022 & --\\
Russia & 1995--2022 & --\\
Saudi Arabia & 2002--2022 & --\\
Senegal & 2014--2022 & --\\
Serbia & 1997--2022 & --\\
Slovakia & 1992--2022 & --\\
Slovenia & 1995--2022 & --\\
South Africa & 1995--2022 & --\\
South Korea & 1970--2022 & --\\
Spain & 1995--2022 & --\\
Sweden & 1950--2022 & --\\
Switzerland & 1990--2022 & --\\
Trinidad \& Tobago & 1999--2022 & --\\
Tunisia & 1992--2022 & --\\
Turkey & 2009--2022 & --\\
USA & 1970--2022 & 1870--1969\\
Ukraine & 1989--2022 & --\\
United Kingdom & 1970--2022 & 1855--1969\\
Uruguay & 2016--2022 & --\\
Uzbekistan & 2010--2022 & --\\
Vanuatu & 2001--2022 & --\\
Venezuela & 1997--2022 & --\\
\bottomrule
\end{tabular}
\end{minipage}
}
\end{table}

==> tables/tbl-wid_c_table.tex <==
\begin{table}[pos=h]
\caption{Regression of $- \Delta c^*$ and $\Delta q_c$ on $\Delta g(K)$ (Screen = 0.01). $H_0 \text{ per thrift theory: } \Delta g(K) \cong -\Delta c^* \& \Delta q_c \cong 0$}
\centering
\begin{tabularx}{\columnwidth}{lcc}
   \toprule
                                               & $-\Delta c^*$   & $\Delta q_c$ \\    
   \midrule 
   Regression of value shown on $\Delta g(K)$  & -0.3760$^{***}$ & 1.376$^{***}$\\   
                                               & (0.1055)        & (0.1055)\\   
    \\
   Observations                                & 1,548           & 1,548\\  
   R$^2$                                       & 0.53993         & 0.88294\\  
   Within R$^2$                                & 0.31853         & 0.86226\\  
    \\
   Year fixed effects                          & $\checkmark$    & $\checkmark$\\   
   Country fixed effects                       & $\checkmark$    & $\checkmark$\\   
   \bottomrule
\end{tabularx}
   \label{tbl-wid_c_table}
\end{table}
